Investigation of Electroweak Production of the Top Quark at the LHC

This thesis presents a study of the prospects of measuring electroweak production of the top quark at the LHC. The study of the top quark is a highly topical subject as we expect significant numbers of top quarks at the LHC which will enable us to conduct precision measurements of the properties of the top. The t-channel "single top" is a relatively rare mode of top production but with it we can probe the spin structure of the Wtb vertex in the weak interaction at an unprecedented energy scale through the measurement of the top polarisation. Analysis strategies and computing tools were developed and tested extensively. The study was performed using the signal and background events modelled with Monte Carlo generators, many of which have been newly developed for the LHC analyses. Full and fast simulation of the ATLAS detector was performed to obtain realistic estimates of the sensitivity of the measurements. A new fully fledged analysis framework, "EventView" was developed for the ATLAS collaboration to process these data at the first level of analysis. Parameterised vertex tagging was developed to estimate the level of background for this analysis and a maximum likelihood fit was used for the precise extraction of the top polarisation. In the high energy hadronic environment at the LHC, the estimation of possible systematic errors, both experimental and theoretical, needs to be carefully considered. Important elements of the systematic errors were investigated and the main contributions were evaluated.

==> Abstract.tex <==
%\begin{abstract}
This thesis presents a study of the prospects of measuring electroweak production of the top quark at the LHC. The study of the top quark is a highly topical subject as we expect significant numbers of top quarks at the LHC which will enable us to conduct precision measurements of the properties of the top.  The t-channel ``single top'' is a relatively rare mode of top production but with it we can probe the spin structure of the Wtb vertex in the weak interaction at an unprecedented energy scale through the measurement of the top polarisation.

Analysis strategies and computing tools were developed and tested extensively. The study was done using the signal and background events modelled with Monte Carlo generators, many of which have been newly developed for the LHC analysis. Full and fast simulation of the \ATLAS\ detector were performed to obtain realistic estimates of the sensitivity of the measurements. A new fully fledged analysis framework, ``\EventView'' was developed for the \ATLAS\ collaboration to process these data at the first level of analysis. Parameterised vertex tagging was used to estimate the level of background for this analysis and multi variable discriminant was constructed to reject them. A kinematic fit of the event reconstruction and a maximum likelihood fit were used for the precise extraction of the top polarisation.

In the high energy hadronic environment at the LHC, the estimation of possible systematic errors, both experimental and theoretical, need to be carefully considered. Important elements of the systematic errors were investigated and the main contributions were evaluated.
%\end{abstract}



==> Conclusion.tex <==

In this thesis, a technique was developed for the measurement of single top polarisation. W plus jets background was estimated using a transfer rate function b-tagging and the top quark was reconstructed using a W mass constraint. The single top polarisation was measured using a binned maximum likelihood method with template histograms. Different signal models and analysis strategies were considered.

The expected statistical error for the polarisation measurement is $\sim 10\%$ at $1\mathrm{fb}^{-1}$ and $\sim 1\%$ at $30\mathrm{fb}^{-1}$though evaluation of systematics remains to be an important issue to be addressed. Same indication of model dependency was observed from using different MC generators and detailed investigation need to confirm the details of such an effect. Other systematics include understandings of ISR/FSR and PDF uncertainties which affects the event selection efficiency.

Improvements on the technique are being developed including smoothing of the template distribution for more stable extraction of the polarisation measurement. A kinematic fit using extra event constraints such as top mass is also under consideration. Improved methods are required for the rejection of $t\bar{t}$ events and multi variable discrimination techniques may be useful for this purpose. Methods of estimating backgrounds such as W plus jets and QCD from data must be established to correctly account for the data in the signal region.

==> Preface.tex <==
\chapter*{Preface}
\begin{quote}
Physicists have been convinced that the top quark must exist since 1977, when its partner, the bottom quark, was discovered. Little did they know it would be nearly two decades before the top was finally found.

The W and Z particles were discovered in 1983 and at that time, and for some years subsequently, the data were not precise enough to be sensitive to virtual top effects. In the late 1980s and early 1990s, LEP at CERN and SLC at Standford began to produce new and highly accurate data which did allow increasingly precise predictions to be made for the top quark mass, $m_t$. Thus, a kind of race began, between experimentalists searching for the real top and theorists fitting ever more precise data to get tighter and tighter limits on $m_t$ from its virtual effects.

In fact, by the time of the actual experimental discovery of the top quark, the experimental error in $m_t$ was just about the same as the theoretical one. Thus, in their May 1994 review of the electroweak theory, Langacker and Erler gave the result of a fit to all electroweak data as

\[ m_t=169 \pm ^{16}_{18} \pm ^{17}_{20} ~\mathrm{GeV} \]

the central figure and first error being based on Higgs mass of 300GeV, while the second error is from the Higgs mass dependency. At about the same time, Ellis et al (1994) gave the extraordinarily precise value

\[ m_t = 162\pm 9 ~ \mathrm{GeV}\]

without any assumption for $m_H$.

A month or so earlier, the CDF collaboration (Abe et al 1994a, b) announced 12 events consistent with the hypothesis of production of a \ttbar\ pair and, on this hypothesis, the mass was found to be 

\[ m_t = 174\pm10 \pm^{13}_{12} ~ \mathrm{GeV} \]

and this was followed by nine similar events from D0. By February 1995 both groups had amassed more data and the discovery was announced. The 2007 experimental value for $m_t$ is $170.9 \pm 1.1 (\mathrm{stat}) \pm 1.5 (\mathrm{syst})~\mathrm{GeV}$ as compared to the value predicted by fits to the electroweak data of $175.3\pm4.4$ GeV. This represents an extraordinary triumph for both theory and experiment. It is surely remarkable how the quantum fluctuations of a yet-to-be detected new particle could pin down its mass so precisely. It seems hard to deny that Nature has, indeed made use of the subtle intricacies of a renormalisable, spontaneously broken, non-Abelian chiral gauge theory.
\end{quote}
\begin{flushright}
--I. J. R. Aitchison and A. J. G. Hey
\end{flushright}



